Controllable Dynamic Appearance for Neural 3D Portraits

Recent advances in Neural Radiance Fields (NeRFs) have made it possible to reconstruct and reanimate dynamic portrait scenes with control over head-pose, facial expressions and viewing direction. However, training such models assumes photometric consistency over the deformed region e.g. the face must be evenly lit as it deforms with changing head-pose and facial expression. Such photometric consistency across frames of a video is hard to maintain, even in studio environments, thus making the created reanimatable neural portraits prone to artifacts during reanimation. In this work, we propose CoDyNeRF, a system that enables the creation of fully controllable 3D portraits in real-world capture conditions. CoDyNeRF learns to approximate illumination dependent effects via a dynamic appearance model in the canonical space that is conditioned on predicted surface normals and the facial expressions and head-pose deformations. The surface normals prediction is guided using 3DMM normals that act as a coarse prior for the normals of the human head, where direct prediction of normals is hard due to rigid and non-rigid deformations induced by head-pose and facial expression changes. Using only a smartphone-captured short video of a subject for training, we demonstrate the effectiveness of our method on free view synthesis of a portrait scene with explicit head pose and expression controls, and realistic lighting effects. The project page can be found here: http://shahrukhathar.github.io/2023/08/22/CoDyNeRF.html

==> scrap.tex <==
\subsection{The lighting model}

The outgoing radiance at any point \(\xbf\), for a particular articulation of facial expression and head-pose, \(\beta_{\text{e,p}}\) is given by the rendering equation as follows:

\begin{smequation}
    L_r\left(\mathbf{x}, \omegabf_o, \beta_{\text{e,p}}\right)=\int_{\omega_i} \rhobf\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)\left(\mathbf{n} \cdot \omegabf_i\right) L_i\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i
    \label{eq:rend_eq}
\end{smequation}
where, \(\rhobf\) is the articulation dependent BRDF, \(\nbf\) is the normal at \(\xbf\) and \(\omega_i, \omega_o\) are the incoming and outgoing ray directions respectively. Next, we assume the BRDF be decomposed into a diffuse and specular component:

\begin{smequation}
    \rhobf\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right) = k_{d} + k_{s}\times \rhobf'\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)
\end{smequation}
 where, \(k_{d}\) and \(k_{s}\) are appropriately chosen normalization constants. The rendering equation now becomes
 
\begin{smequation}
\begin{split}
     &L_r\left(\mathbf{x}, \omegabf_o, \beta_{\text{e,p}}\right)=\int_{\omega_i} \left(k_{d} + k_{s}\rhobf'\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)\right)\left(\mathbf{n} \cdot \omegabf_i\right) L_i\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i\\
     &= \int_{\omega_i}k_{d}\left(\mathbf{n} \cdot \omegabf_i\right) L_i\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i \\
     &\quad\quad\quad + \int_{\omega_i} k_{s}\rhobf'\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)\left(\mathbf{n} \cdot \omegabf_i\right) L_i\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i
\end{split}
    \label{eq:rend_eq_sp}
\end{smequation}
we now make another simplifying assumption; cast shadows attenuates incident light at a point by a constant factor in all directions\footnote{Shadow edges are the only exception}. Thus, we can write \(L_i\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) = S(\mathbf{x},\beta_{\text{e,p}} )L_i^{'}\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right)\). The rendering equation now becomes:
\begin{smequation}
\begin{split}
     &L_r\left(\mathbf{x}, \omegabf_o, \beta_{\text{e,p}}\right)= \int_{\omega_i}k_{d}\left(\mathbf{n} \cdot \omegabf_i\right) S(\mathbf{x},\beta_{\text{e,p}} )L_i^{'}\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i \\
     &\quad\quad\quad + \int_{\omega_i} k_{s}\rhobf'\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)\left(\mathbf{n} \cdot \omegabf_i\right)S(\mathbf{x},\beta_{\text{e,p}} )L_i^{'}\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i\\
     &= S(\mathbf{x},\beta_{\text{e,p}} )\int_{\omega_i}k_{d}\left(\mathbf{n} \cdot \omegabf_i\right) L_i^{'}\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i \\
     &\quad\quad\quad + S(\mathbf{x},\beta_{\text{e,p}} )\int_{\omega_i} k_{s}\rhobf'\left(\mathbf{x}, \omegabf_i, \omegabf_o, \beta_{\text{e,p}}\right)\left(\mathbf{n} \cdot \omegabf_i\right) L_i^{'}\left(\mathbf{x}, \omegabf_i, \beta_{\text{e,p}}\right) \mathrm{d} \omega_i
\end{split}
    \label{eq:rend_eq_sp_2}
\end{smequation}
We approximate the first term using spherical harmonics along with an articulation-dependent albedo predicted by an MLP, the second integral with another MLP dependent on the reflection vector and the shading attenuation with a third MLP. The final radiance is given as follows:

\begin{smequation}
\begin{split}
    &L_r\left(\mathbf{x}, \omegabf_o, \beta_{\text{e,p}}\right)= MLP_{S}(\mathbf{x},\beta_{\text{e,p}} )\times MLP_{\text{albedo}}(\mathbf{x},\beta_{\text{e,p}})\times\Phi(\mathbf{n}(\xbf))\\
    &\quad\quad\quad + MLP_{S}(\mathbf{x},\beta_{\text{e,p}}) \times MLP_{\text{specular}}(\mathbf{x},\beta_{\text{e,p}},\omegabf_o )
\end{split}
\end{smequation}

==> teaser.tex <==
\centering
\includegraphics[width=0.99\linewidth]{Teaser_v4.pdf}
%\captionof{figure}{Our method, \MethodName, enables the creation of reanimatable Neural 3D portraits from a video captured under challenging lighting conditions with a smartphone. Through a novel dynamic canonical appearance modeling method, \MethodName is not only able to faithfully reconstruct the appearance (including lighting) in novel views (first column), but also modeling the varying illumination effect with controllable facial expressions and head-poses (column 2-4).%On the left, we show the results of \MethodName for different head-poses, facial expressions and viewing directions.}
\captionof{figure}{\small{Our method, \MethodName, enables the creation of reanimatable Neural 3D portraits from a video captured under challenging lighting conditions with a smartphone (column (a)). \MethodName uses a novel dynamic canonical appearance model (column (b),  discussed in \sect{dyconnerf}) to predict illumination effects during reanimation and novel view synthesis (column (c)). Compared to prior work \cite{rignerf}, \MethodName's prediction of illumination effects is more accurate and its renders of articulated facial expression and head-pose are of higher quality (column (d)).}}%On the left, we show the results of \MethodName for different head-poses, facial expressions and viewing directions.}
%\figcaption{{}
